Functors from the infinitary model theory of modules and the Auslander-Gruson-Jensen 2-functor

We define the notion of a $\lambda$-definable category, a generalisation of the notion of definable category from the model theory of modules. Let ${\cal C}$ be a $\lambda$-accessible additive category. We characterise the additive functors ${\cal} C\to{\mathrm Ab}$ which preserve $\lambda$-directed colimits and products, by showing that they are the finitely presented functors determined by a morphism between $\lambda$-presented objects (the same result appears, for the case $\lambda=\omega$, in \cite{prest2011}, but we give a proof for any infinite regular cardinal $\lambda$). We remark that \cite{arb} shows that every $\lambda$-definable subcategory of ${\cal C}$ is the class of zeroes of some set of such functors, thus obtaining a $\lambda$-ary generalisation of the finitary ($\lambda = \omega$) result from the finitary model theory of modules. We show that, to analyse the $\lambda$-ary model theory of a locally $\lambda$-presentable additive category ${\cal C}$, it is sufficient to consider \emph{finitary} pp formulas in the language of right ${\mathrm{Pres}_\lambda}{\cal C}$-modules, where ${\mathrm{Pres}_\lambda}{\cal C}$ is the category of $\lambda$-presented objects of ${\cal C}$, with the caveat that these pp formulas are interpreted among right ${\mathrm{Pres}_\lambda}{\cal C}$-modules which preserve $\lambda$-small products. In particular, for an additive category ${\cal R}$ with $\lambda$-small products (e.g. ${\cal R}={\mathrm{Pres}_\lambda}{\cal C}^{\mathrm op}$ for ${\cal C}$ a $\lambda$-presented additive category), the $\lambda$-accessible functors ${\cal N}\to{\mathrm Ab}$ which preserve products are precisely the finitely accessible functors ${\cal R}{\mathrm Mod}\to{\mathrm Ab}$ which preserve products, restricted to ${\cal N}$, where ${\cal N}\subseteq{\cal R}{\mathrm Mod}$ is the category of left ${\cal R}$-modules which preserve $\lambda$-small products.

==> elem-cogens.tex <==
\begin{defn}
    Let $\Q$ be an additive category with products.
    An object $Q\in\Q$ is called an \textbf{elementary cogenerator} if every object of $\Q$ is a split subobject of some power of $Q$.
    (When $\Q$ has split idempotents, ``split subobject'' may be replaced by ``summand''.)
\end{defn}

\begin{lem}
    \thlabel{Qstuff}
    Suppose $\Q$ has products and let $Q\in\Q$ be given.
    The following are equivalent:
    \begin{enumerate}
        \item\label{itm:a} $Q$ is an elementary cogenerator of $\Q$.
        \item\label{itm:b} For any functor $F:\Q\to\Ab$ which preserves products, there is an epimorphism $\Hom_\Q(Q^{FQ},-)\to F$.
        \item\label{itm:c} For any object $A\in\Q$, the canonical map $A\to Q^{\Hom_\Q(A,Q)}$ is a split monomorphism.
    \end{enumerate}

\end{lem}
\begin{proof}
    $\ref{itm:a}\implies\ref{itm:b}$: Let a natural transformation $\alpha:F\to G$ be given, where $G$ also preserves products.
    It is easy to show that
    \begin{displaymath}
        \alpha_Q=0\iff \alpha = 0.
    \end{displaymath}
    For each $y\in FQ$ let $\pi_y:Q^{FQ}\to Q$ be the projection.

    Let $\phi:\Hom_\C(Q^{FQ},-)\to F$ be the corresponding natural transformation to the element $x\in F(Q^{FQ})$ such that $(F \pi_y)x=y$ for each $y\in FQ$.
    Then
    \begin{displaymath}
        \phi_Q(\pi_y)= (F\pi_y)x =y
    \end{displaymath}
    for each $y\in FQ$.

    We have $\alpha\phi=0\iff\alpha=0$, since for any $y\in FQ$,
    \begin{displaymath}
        \alpha_Q(y)=\alpha_Q\phi_Q(\pi_y).
    \end{displaymath}

    Now take the cokernel $G=F/\Img\phi$ of $\phi$.
    By the exactness of products in $\Ab$, $G$ preserves products.
    Take $\alpha:F\to G$ to be the quotient.
    Since $\alpha \phi=0$, $\alpha=0$.
    Therefore $\Img\phi=F$, so $\phi$ is an epimorphism.

    $\ref{itm:b}\implies\ref{itm:c}$: For any $A\in\Q$, $\Hom_\Q(A,-)$ preserves products and the canonical map induces a natural transformation
    \begin{displaymath}
        \alpha:\Hom_\Q(Q^{\Hom_\Q(A,Q)},-)\to\Hom_\Q(A,-).
    \end{displaymath}
    Let $F=\Coker(\alpha)$.
    Then $F$ preserves products and by~\ref{itm:b}, if $FQ=0$ then $F=0$.
    However, $\alpha_Q$ is an epimorphism since, for any $f\in\Hom_\Q(A,Q)$, $\alpha(\pi_f)=f$, so $F=0$ and $\alpha$ is an epimorphism.
    Thus the canonical map is a split monomorphism.

    $\ref{itm:c}\implies\ref{itm:a}$: By definition.
\end{proof}

\begin{cor}
    If $\Q$ is an additive category with products and elementary cogenerator, then any functor $\Q\to\Ab$ which preserves products is finitely presented.
\end{cor}
\begin{proof}
    Let $Q$ be the injective cogenerator and let $\phi:\Hom_\Q(Q^{FQ},-)\to F$ be an epimorphism by \thref{Qstuff}\ref{itm:b}.
    If $K=\Ker(\phi)$ then, by the exactness of products, $K$ preserves products.
    Therefore, again by \thref{Qstuff}\ref{itm:b}, there is an exact sequence
    \begin{displaymath}
        \xymatrix{\Hom_\Q(Q^{KQ},-)\ar[r]&\Hom_\Q(Q^{FQ},-)\ar[r]^-\phi&F\ar[r]&0}
    \end{displaymath}
\end{proof}

\begin{cor}
    If $\Q$ has an elementary cogenerator then $\fp{\Q,\Ab}$ is abelian and $\Q$ has weak cokernels.
\end{cor}
\begin{proof}
    Suppose $\Q$ has an elementary cogenerator.
    The finitely presented functors $\Q\to\Ab$ are precisely the functors which preserve products.
    Since products are exact in $\Ab$, the category of functors $\Q\to\Ab$ which preserve products has object-wise kernels and cokernels, so it is clearly abelian.
    By \thref{aus}, $\Q$ has weak cokernels.
\end{proof}

\begin{rmk}
    Suppose $\Q$ has an elementary cogenerator $Q$.
    The statements in this section refer to products in $\Q$, and functors $\Q\to\Ab$ which preserve them.
    It is clear that, to make the proofs go through, we actually only needed all powers $Q^I$ to exist, and to consider functors preserve such powers.
    From this we see that: \emph{If a functor $F:\Q\to\Ab$ preserves all powers of $Q$, then it preserves all products} (since it is finitely presented by the proof of \thref{Qstuff}$\ref{itm:a}\implies\ref{itm:b}$).
\end{rmk}

\begin{ex}
    Let $K$ be a field and let $\C= K\Mod$.
    For any full subcategory $\Q\subseteq\C$ closed under products, every non-zero object of $\Q$ is an elementary cogenerator for $\Q$, and so every functor $\Q\to\Ab$ which preserves products is finitely presented.
    It follows that such functors are of the form $\Hom(M,-)|_\Q$ for some $M\in K\Mod$, or equivalently that they are powers of the forgetful functor $\Q\to\Ab$.
    Some of these examples lack split idempotents, e.g. $\Q=\setc{V\in K\Mod}{\dim V\neq 1}$.
\end{ex}
